TempLe: Learning Template of Transitions for Sample Efficient Multi-task RL

Transferring knowledge among various environments is important to efficiently learn multiple tasks online. Most existing methods directly use the previously learned models or previously learned optimal policies to learn new tasks. However, these methods may be inefficient when the underlying models or optimal policies are substantially different across tasks. In this paper, we propose Template Learning (TempLe), the first PAC-MDP method for multi-task reinforcement learning that could be applied to tasks with varying state/action space. TempLe generates transition dynamics templates, abstractions of the transition dynamics across tasks, to gain sample efficiency by extracting similarities between tasks even when their underlying models or optimal policies have limited commonalities. We present two algorithms for an "online" and a "finite-model" setting respectively. We prove that our proposed TempLe algorithms achieve much lower sample complexity than single-task learners or state-of-the-art multi-task methods. We show via systematically designed experiments that our TempLe method universally outperforms the state-of-the-art multi-task methods (PAC-MDP or not) in various settings and regimes.

==> algos/group_alg_new.tex <==
%!TEX root = ../0_aaai_all.tex


\begin{algorithm}[!ht]
   \caption{\mbox{\ourmodtwofull (\ourmodtwo)}}
   \label{alg:group}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} $\hat{\tau}$; $\epsilon$; $\gamma$; $\thressm$; $\threslg$ (same as Algorithm~\ref{alg:main});\\
   number of tasks in the first phase $T_1$; number of models $C$; model error tolerance $\eta$
   \STATE {\bfseries Output:} Near-optimal policies $\{\pi_t\}_{t=1,2,\cdots}$
   \STATE Initialize the \patname group set $\patset$, the \patname visit set $\patvisset$, and the MDP group set $\mdpset$ as empty
   % \STATE Set the value of $\thressm$ and $\threslg$ according to Equation~\ref{eq:thres}~\fh{delete this, as it is shown in algorithm 1 already?}
   \FOR{$t \gets 1,2,\cdots, T_1$}
    \STATE Receive a task $M_t$ 
    \STATE Run Algorithm xx
   \ENDFOR
   \STATE Cluster the $T_1$ tasks into $\hat{C} \leq C$ groups (store in $\mdpset$).
   \STATE For each model group $c$, compute \patnames $\pattern_{s,a,c}$ and corresponding permutations $\permut_{(s,a,c)}$ for all $s,a$
   \FOR{$t \gets T_1+1, T_1+2, \cdots$}
    \STATE Receive a task $M_t$ 
    \STATE Initialize the model score $u(c)=\eta, \forall c \in \mdpset$
    \STATE Run Algorithm xx, check the following condition for every step
    \IF{the \patname of $(s,a)$ is identified}
    \STATE $u(c) \gets u(c) - 1$, $\forall c\in\mdpset$ s.t $\pattern_{(s,a,c)}\neq \pattern_{(s,a)}$ or the permutation $\permut_{(s,a,c)}\neq \permut_{(s,a)}$
    \ENDIF
    \IF{there is only 1 MDP group $c\in \mdpset$ s.t. $u(c)>0$}
    \STATE Incorporate all counts of $c$ to the current task~\fh{could you use $N$ again?}
    \ENDIF
   \ENDFOR 
\end{algorithmic}
\end{algorithm}


==> algos/main_alg_old.tex <==
%!TEX root = ../0_icml2020_multitaskrl_main.tex

% \begin{algorithm}[!ht]
% \DontPrintSemicolon
% \caption{OurAlgorithm1}
% \label{alg:main}
%   \Input{$S$; $A$; $\tau$; $\epsilon$; $\gamma$}
%   % Episode number $T$; horizon $H$; error tolerance $\epsilon$; 
%   % known threshold $m$; completion fraction $\fraction$; walking parameter $\beta$} 
%   \Output{Near-optimal policies $\{\pi_t\}_{t=1,2,\cdots}$}
%   Initialize the pattern group $\patset$ as empty. \;
%   Set the value of $\thressm$ and $\threslg$ according to \yc{eq} \;
%   \For{$t \gets 1,2,\cdots$}{
%     Receive a task $M_t$ \;
%     Set $A(s,a)=\thressm$ for all $ s \in \states, a \in \actions$
%     $\pi \gets \Sin(M_t, A)$ \;
%     \For{$h \gets 1,2,\cdots,H$}{
%       $a_h \gets \pi(s_h)$ \;
%       Take action $a_h$, get $s_{h+1}$ and $r_h$ \;
%       \Up($s_h, a_h, s_{h+1}, r_h$)\;
%     }
%     % \If{any state-action pair $(s,a)$ is $\tau$-known{\fh{undefined}}}{
%     %     \eIf{no $\pattern \in \patset$ is $\tau$-close to $\theta(s,a)$}{
%     %       Add $\permut_{(s,a)}(\theta(s,a))$ to $\patset$ \;
%     %     }{
%     %       Find $\pattern_i \in \patset$ which is $\tau$-close to $\theta(s,a)$ \;
%     %       Add the visits to the current s-a pair $o(s,a)$ {\fh{undefined}}to $\patviss_i$; set $o(s,a)=\patviss_i$.
%     %     }
%     %     Set the known threshold of $(s,a)$ to $\mathcal{O}(\frac{V_{\max}^2}{(\epsilon^2 (1-\gamma)^2})$. \;{\fh{requires explanation in the main body of the paper}}
%     % }
%     % \If{any s-a pair is $(\frac{V_{\max}^2}{(\epsilon^2 (1-\gamma)^2})$-known}{
%     %     Update policy \;{\fh{how?}}
%     % }
%   }
%   \Fn{\Up($s,a,s^\prime,r$)}{
%     Update $n(s,a),n(s,a,s^\prime), r(s,a)$ \;
%     \If{$n(s,a)\geq A(s,a) \wedge A(s,a) = \thressm$}{
%       $\tilde{\pattern} \gets \Pa(\hat{p}(s,a),\hat{r}(s,a))$ \;
%       \eIf{no $\pattern \in \patset$ is $\tau$-close to $\tilde{\pattern}$}{
%         Add $\tilde{\pattern}$ to $\patset$ with visits \;
%       }{
%         Find the closest pattern $\pattern^*$ to $\tilde{\pattern}$ \;
%         Add visits of $(s,a)$ to $\pattern^*$ \;
%         Incorporate all visits of $\pattern^*$ to $(s,a)$
%       }
%       $A(s,a) \gets \threslg$ \;
%     }
%     \If{$n(s,a)\geq A(s,a) \wedge A(s,a) = \threslg$}{
%       $\pi \gets \Sin(M_t, A)$
%     }
%   }
% \end{algorithm}


\alglanguage{pseudocode}
\begin{algorithm}[!htbp]
   \caption{\ourmodfull (\ourmod)}
   \label{alg:main}
   \hspace*{\algorithmicindent} \textbf{Input:} 
   user-specified \patname gap $\hat{\tau}$; error tolerance $\epsilon$; discount factor $\gamma$; fully known threshold $\threslg$; roughly known threshold $\thressm$ \\
   \hspace*{\algorithmicindent} \textbf{Output} 
   Near-optimal policies $\{\pi_t\}_{t=1,2,\cdots}$
\begin{algorithmic}[1]
%<<<<<<< HEAD
   \State Initialize empty \patname group set $\patset$ and the \patname visit set $\patvisset$    \For{$t \gets 1,2,\cdots$}
    \State Receive a task $M_t$
    \State Set $A(s,a)\leftarrow \thressm$ as thresholds, initialize visits $n(s,a), n(s,a,s^\prime),R(s,a)$ to 0, $\forall (s, s^\prime,a) \in (\states, \states, \actions)$
    \State Initialize $\pi$ as a random policy 
    \For{$h \gets 1,2,\cdots,H$}
     % \STATE Action $a_h \gets \pi(s_h)$ 
      \State Take action $a_h \gets \pi(s_h)$, get $s_{h+1}$ and $r_h$
      \State $n(s_h,a_h) \leftarrow n(s_h,a_h)+1$
       \State $n(s_h,a_h,s_{h+1}) \leftarrow n(s_h,a_h,s_{h+1})+1$
        \State $R(s_h,a_h)\leftarrow R(s_h,a_h)+r_h$
      \If{ $ A(s_h,a_h) = \thressm $ \textbf{and}  $ n(s_h,a_h) = \thressm $}
      \Comment{{\scriptsize{\patname identification with the small threshold}}}
      \State $\patvisp_{\tilde{\pattern}}\gets descending(\bm{n}(s_h,a_h,\cdot))$
        \State $\patvisr_{\tilde{\pattern}}\gets R(s_h,a_h)$
        \State $\tilde{\pattern} \gets (\frac{\patvisp_{\tilde{\pattern}}}{n(s_h,a_h)}, \frac{\patvisr_{\tilde{\pattern}}}{n_(s_h,a_h)})$
        \If{no $\pattern \in \patset$ is $\hat{\tau}$-close to $\tilde{\pattern}$}
          % \COMMENT{Initialize a new \patname}
          % \State \tcb{\# Initialize a new \patname}
          \State Add $\tilde{\pattern}$ to $\patset$,
          %\State $\patvisp_{\tilde{\pattern}}=desc(\bm{n}(s_h,a_h,\cdot))$
          %\State $\patvisr_{\tilde{\pattern}}=R(s_h,a_h)$
      $\patvis_{\tilde{\pattern}}=(\patvisp_{\tilde{\pattern}}, \patvisr_{\tilde{\pattern}})$ to $\patvisset$
%=======
%   \State Initialize the \patname group set $\patset$ and the \patname visit set $\patvisset$ as empty. 
%   \For{$t \gets 1,2,\cdots$}
%    \State Receive a task $M_t$ 
%    \State Initialize the threshold table $A$: set $A(s,a)=\thressm$ for all $ s \in \states, a \in \actions$
%    \State Initialize visits $n(s,a), n(s,a,s^\prime), R(s,a)$, for all $ s, s^\prime \in \states, a \in \actions$
%    \State Compute a policy $\pi$ using visits by RMax
%    \For{$h \gets 1,2,\cdots,H$}
%     % \STATE Action $a_h \gets \pi(s_h)$ 
%      \State Take action $a_h$ according to $\pi(s_h)$, get $s_{h+1}$ and $r_h$ 
%      \State Update $n(s_h,a_h), n(s_h,a_h,s_{h+1}),R(s_h,a_h)$
%      \If{$ n(s,a)\geq A(s,a) $ \textbf{and} $ A(s,a) = \thressm $}
%        \State $\tilde{\pattern} \gets (desc(\bm{n}(s,a,\cdot)/n(s,a)),\hat{r}(s,a))$
%        \If{no $\pattern \in \patset$ is $\hat{\tau}$-close to $\tilde{\pattern}$}
%          % \COMMENT{Initialize a new \patname}
%          % \State \tcb{\# Initialize a new \patname}
%          \State $\patvisp_{\tilde{\pattern}}=desc(\bm{n}(s,a,\cdot))$
%          \State $\patvisr_{\tilde{\pattern}}=R(s,a)$
%          \State Add $\patvis_{\tilde{\pattern}}=(\patvisp_{\tilde{\pattern}}, \patvisr_{\tilde{\pattern}})$ to $\patvisset$
%          \State Add $\tilde{\pattern}$ to $\patset$
%>>>>>>> db63217899b4657f34cb94249810cea1d32e302b
        \Else
          \State Find the closest \patname $\pattern^*$ to $\tilde{\pattern}$ 
          \State \Call{\patname-update}{$\pattern^*, \patvis_{\pattern^*}, \bm{n}(s_h,a_h,\cdot), R(s_h,a_h)$}
          \State {\small{\Call{visits-update}{$\patvis_\pattern^*, n(s_h,a_h) ,\bm{n}(s_h,a_h,\cdot), R(s_h,a_h)$}}}
          % \State \tcb{\# Add current experience to \patname}
          % \State $\patvis_{\pattern^*} \leftarrow \patvis_{\pattern^*} + (desc(\bm{n}(s,a,\cdot)),R(s,a))$
          % \State $\pattern^* \leftarrow (\patvisp_{\pattern^*}/\sum \patvisp_{\pattern^*}, \patvisr_{\pattern^*}/\sum \patvisp_{\pattern^*})$
          % \State \tcb{\# Add \patname experience to current task}
          % \State Get the permutation $\permut$ that orders $\bm{n}(s,a,\cdot)$ descendingly
          % \State $\bm{n}(s,a,\cdot) \leftarrow \bm{n}(s,a,\cdot) + \permut^{-1}(\patvisp_{\pattern^*})$,\\ $R(s,a) \leftarrow R(s,a) + \patvisr_{\pattern^*}$, \\ $n(s,a) \leftarrow n(s,a) + \sum_{s^\prime} \bm{n}(s,a,s^\prime)$
           % \fh{Update $\pattern^*\leftarrow [\frac{n_{\pattern^*}(s,a,s_1)}{n_{\pattern^*}(s,a)},\ldots,\frac{n_{\pattern^*}(s,a,s_S)}{n_{\pattern^*}(s,a)}]$}
        \EndIf
        \State Update threshold $A(s_h,a_h) \gets \threslg$ 
      \EndIf
      \If{$ A(s_h,a_h) = \threslg $ \textbf{and} $ n(s_h,a_h) = m $}\quad\quad
      \Comment{{\scriptsize{policy update with the regular threshold}}}
        \State Update $\pi$ using visits by RMax
      \EndIf
    \EndFor
    \For{all $(s,a) \in (\states, \actions)$ with identified \patname $\pattern_{(s,a)}$}
      \State \Call{\patname-update}{$\pattern_{(s,a)}, \patvis_{\pattern_{(s,a)}}, \bm{n}(s,a,\cdot), R(s,a)$}
      % \State\tcb{\# Add the rest current experience to \patname}
      % \State$\patvis_{\pattern_{(s,a)}} \leftarrow \patvis_{\pattern_{(s,a)}} + (desc(\bm{n}(s,a,\cdot)),R(s,a))$
      % \State$\pattern_{(s,a)} \leftarrow (\patvisp_{\pattern_{(s,a)}}/\sum \patvisp_{\pattern_{(s,a)}}, \patvisr_{\pattern_{(s,a)}}/\sum \patvisp_{\pattern_{(s,a)}})$
    \EndFor 
    \EndFor
    \Function{\patname-update}{$\pattern, \patvis_\pattern, \bm{n}, R$}
      \State $\patvis_{\pattern} \gets \patvis_{\pattern} + (descending(\bm{n}),R)$
      \State $\pattern \gets (\frac{\patvisp_{\pattern}}{\lVert \patvisp_{\pattern} \rVert_{\ell_1}}, \frac{\patvisr_{\pattern}}{\lVert \patvisp_{\pattern} \rVert_{\ell_1}})$
    \EndFunction
    \Function{visits-update}{$\patvis_\pattern, n, \bm{n}$}\fh{R missing}
      \State Get the permutation $\permut$ that orders $\bm{n}$ descendingly
      \State $\bm{n} \gets \bm{n} + \permut^{-1}(\patvisp_{\pattern})$, $n \gets n + \lVert \bm{n} \rVert_{\ell_1}$~\fh{shouldn't $n$ be $\lVert \bm{n} \rVert_{\ell_1}$?}
      \State $R \gets R + \patvisr_{\pattern}$ 
    \EndFunction
\end{algorithmic}
% \begin{algorithmic}[1]
%    \STATE{\bfseries Function} Update($s,a,s^\prime,r$)
%    \STATE Update $n(s,a),n(s,a,s^\prime), r(s,a)$ 
%     \IF{$n(s,a)\geq A(s,a) \wedge A(s,a) = \thressm$}
%       \STATE $\tilde{\pattern} \gets Patternize(\hat{p}(s,a),\hat{r}(s,a))$ 
%       \IF{no $\pattern \in \patset$ is $\tau$-close to $\tilde{\pattern}$}
%         \STATE Add $\tilde{\pattern}$ to $\patset$ with visits 
%       \ELSE
%         \STATE Find the closest pattern $\pattern^*$ to $\tilde{\pattern}$ 
%         \STATE Add visits of $(s,a)$ to $\pattern^*$ 
%         \STATE Incorporate all visits of $\pattern^*$ to $(s,a)$
%       \ENDIF
%       \STATE $A(s,a) \gets \threslg$ 
%     \ENDIF
%     \IF{$n(s,a)\geq A(s,a) \wedge A(s,a) = \threslg$}
%       \STATE $\pi \gets SingleRMax(M_t, A)$
%     \ENDIF
% \end{algorithmic}
\end{algorithm}

==> algos/patternize.tex <==
%!TEX root = ../0_icml2020_multitaskrl_main.tex

% \begin{algorithm}[!ht]
% \DontPrintSemicolon
% \caption{Patternize}
% \label{alg:pattern}
%   \Input{Transition probability $p\in \mathbb{R}^{S}$; reward $r$}
%   \Output{The corresponding pattern $g$ and permutation $\permut$}
%   Initialize the pattern group $\patset$ and pattern visits group $\patvisset$. \;
  
% \end{algorithm}

\begin{algorithm}[tb]
   \caption{Patternize}
   \label{alg:pattern}
\begin{algorithmic}
   \STATE {\bfseries Input:} Transition probability $p\in \mathbb{R}^{S}$; reward $r$
   \STATE {\bfseries Output:} The corresponding pattern $\pattern$ and permutation $\permut$
   \STATE Initialize $\pattern$ and $\permut$ as empty lists
   \STATE Set all elements of $p$ to be active
   \REPEAT
   \STATE $a \gets$ the largest active element of $p$
   \STATE $i \gets$ the smallest index of $a$ in $p$
   \STATE Append $a$ to $\pattern$, and $i$ to $\permut$
   \STATE Set the $i-$th bit of $p$ to be inactive
   \UNTIL{$p$ only has zero-value active elements}
\end{algorithmic}
\end{algorithm}

==> algos/single.tex <==
%!TEX root = ../0_icml2020_multitaskrl_main.tex


% \begin{algorithm}[!ht]
% \DontPrintSemicolon
% \caption{SingleRMax}
% \label{alg:single}
%   \Input{MDP $M$; threshold map $A$}
%   \Output{Near-optimal policy $\pi$}
%   Compute $Q(s,a)$ for all $s \in \states, a \in \actions$ by \yc{eq}
%   \For{state $s \in \states$}{
%     \eIf{$n(s,a) \geq A[s][a]$ for all $a\in \actions$}{
%       $\pi(s) \gets \mathrm{argmax}_a Q(s,a)$
%     }{
%       $\pi(s) \gets$ the action chosen fewest times
%     }
%   }
% \end{algorithm}

\begin{algorithm}[tb]
   \caption{SingleRMax}
   \label{alg:single}
\begin{algorithmic}
   \STATE {\bfseries Input:} MDP $M$; threshold $\threslg$
   \STATE {\bfseries Output:} Near-optimal policy $\pi$
   \STATE For $\threslg$-known $(s,a)$, compute $\hat{p}(s,a)$ and $\hat{r}(s,a)$ \yc{refer}
   \STATE For non-$\threslg$-known $(s,a)$, compute \yc{refer}
   \STATE Compute $Q(s,a)$ for all $s \in \states, a \in \actions$ by \yc{eq}
   \FOR{state $s \in \states$}
   \IF{$n(s,a) \geq \threslg$ for all $a\in \actions$}
   \STATE $\pi(s) \gets \mathrm{argmax}_a Q(s,a)$
   \ELSE
   \STATE $\pi(s) \gets$ the action chosen fewest times
   \ENDIF
   \ENDFOR
\end{algorithmic}
\end{algorithm}

==> figures/paras/paras_ths_run10.tex <==
% This file was created by tikzplotlib v0.9.0.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.4,0.470588235294118,0.67843137254902}
\definecolor{color1}{rgb}{0.776470588235294,0.443137254901961,0.443137254901961}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.91,0.5)}, anchor=east, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={User-specified Small Thresholds},
xmajorgrids,
xmin=21, xmax=219,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Average Rewards},
ymajorgrids,
ymin=9639.626095, ymax=23627.1234335714,
ytick style={color=black}
]
\addplot [semithick, color0, mark=square*, mark size=3, mark options={solid}]
table {%
30 10275.4214285714
60 10275.4214285714
90 10275.4214285714
120 10275.4214285714
150 10275.4214285714
180 10275.4214285714
210 10275.4214285714
};
\addlegendentry{RMax}
\addplot [semithick, color1, mark=diamond*, mark size=3, mark options={solid}]
table {%
30 22865.485
60 22986.463
90 22991.3281
120 22830.39817
150 22683.250219
180 22201.2146533
210 21700.69625731
};
\addlegendentry{FM-TempLe}
\addplot [semithick, white!36.8627450980392!black, mark=triangle*, mark size=3, mark options={solid}]
table {%
30 14741.805
60 14783.0685
90 14863.49445
120 14471.255115
150 14419.3205805
180 15028.47490635
210 14948.223434445
};
\addlegendentry{FMRL}
\end{axis}

\end{tikzpicture}

